Online Selection of Diverse Committees

Citizens' assemblies need to represent subpopulations according to their proportions in the general population. These large committees are often constructed in an online fashion by contacting people, asking for the demographic features of the volunteers, and deciding to include them or not. This raises a trade-off between the number of people contacted (and the incurring cost) and the representativeness of the committee. We study three methods, theoretically and experimentally: a greedy algorithm that includes volunteers as long as proportionality is not violated; a non-adaptive method that includes a volunteer with a probability depending only on their features, assuming that the joint feature distribution in the volunteer pool is known; and a reinforcement learning based approach when this distribution is not known a priori but learnt online.

==> sections/oldies/old_mdp.tex <==
\section{$p$ is known: constrained MDP strategy} \label{sec:cmdp}

In this section, we assume the 
%candidate 
distribution $p$ is known, and we place ourselves in the limit where we would select a committee of infinite size, and aim to maximize the rate at which candidates are selected, under the constraint that the proportion of accepted candidates per feature value is controlled by $\target$. One advantage of this approximation is that the optimal policy is stationary, thus simple to represent. Moreover, 
as stationary policies can be very well 
parallelized, in the case where 
multiple candidates can be interviewed simultaneously. To apply this approach to the finite-size committee selection problem, one needs to interrupt the agent when $K$ candidates have been selected. We showcase a high probability bound of $O(\sqrt{1/K})$ on the representation loss, which guarantees that for large enough values of $K$, the resulting committee is representative. 



\subsection{Our model} 
%We now formalize our committee selection problem as a simple constrained MDP in which actions do not impact the next state. 
Fundamentally, our problem could be seen as a contextual bandit with stochastic contexts $x_t \sim p$ and two actions $a_t = 0$ or $1$. However, the type of constraints incurred by proportional representation are well studied in constrained MDPs (CMDPs) \cite{altman1999constrained}, whereas the contextual bandits literature focused on other constraints (e.g., knapsack constraints \cite{agrawal2016linear}). We show how we can efficiently leverage the CMDP framework for our online committee selection problem.

Formally, we introduce an MDP $M=(\candidateS, \actS, P, r)$, where the set of states is the $d$-dimensional candidate space $\candidateS$, the set of actions is $\actS = \{0, 1\}$, and the (deterministic) reward is $r(x,a) = \indic{a=1}$. 
The transition kernel $P$, which defines the probability to be in state $x'$ given that the previous state was $x$ and the agent took action $a$, is very simple in our case: we simply have $P(x'|x, a) = p(x')$ since candidates are drawn i.i.d regardless of the previous actions and candidates.

We consider the \emph{average reward} setting in which the performance of a policy $\pi:\stateS \times \actS \rightarrow [0, 1]$ is measured by its \emph{gain} $g^{p,\pi}$, defined as:
\begin{align*}
g^{p,\pi}(x) = \lim_{T \rightarrow \infty} \frac{1}{T} \mathbb{E}^{p,\pi}\left[\sum_{t=1}^T r(x_t, a_t) \bigg\vert x_1 = x\right].
\end{align*}
We simply write $g^{p,\pi} := g^{\pi}$ when the underlying transition is $p$ without ambiguity.

We include proportional representation constraints following the framework of CMDPs, where the set of allowed policies is restricted by a set of additional constraints specified by reward functions. In our case, for $i \in \intint{d}, j \in \intint{\size_i}$, we introduce $r_i^j(x, a) = \indic{x_i=j, a=1}$, and let $\cstr_i^j = r_i^j - \target_i^j r$ be the reward function for the constraint indexed by $i,j$. Similarly to the gain, we define ${h_i^j}^\pi = \lim_{T \rightarrow \infty} \frac{1}{T} \mathbb{E}^\pi\left[\sum_{t=1}^T \cstr_i^j(x_t, a_t)\right]$.
The CMDP is defined by:
\begin{align}\label{eq:CMDP-opt1}
    \max_{\pi} \{g^\pi \,| \,\forall i \in \intint{d}, \forall j \in \intint{\size_i}, {h_i^j}^\pi = 0 \}.
\end{align}

Given the simplicity of the transition kernel, and since the MDP is ergodic by the assumption $p > 0$, the gain is constant, i.e. $\forall x \in \candidateS, g^\pi(x) = g^\pi$, and problem \eqref{eq:CMDP-opt1} is well defined. From now on, we only write $g^\pi$ and ${\cstr_i^j}^\pi$.
%Then
The CMDP can be expressed as 
%solved by solving 
the equivalent linear program 
%(LP) 
\cite{altman1999constrained}: 
\begin{equation}\label{eq:CMDP-opt2}
\begin{aligned}
\max_{\mu \in \reals^{\candidateS \times \actS}} \quad & \sum_{x,a}\mu(x,a) r(x,a)  \\
\text{u.c.} \quad & \mu \geq 0, \sum_{x,a} \mu(x,a)  = 1 \\
& \forall x' \in \candidateS, \sum_{x,a} \mu(x,a) P(x'|x, a) = \sum_{a}\mu(x', a) \\
& \forall i,j , \sum_{x,a}\mu(x,a) \cstr_i^j(x,a) = 0.
\end{aligned}
\end{equation}

$\mu : {\candidateS \times \actS} \rightarrow [0, 1]$ is said to be an \emph{occupation measure} \cite{altman1999constrained}, and is defined as: 
\begin{align*}
    \mu(x,a) = \lim_{T\rightarrow \infty}\frac{1}{T}\sum_{t=1}^T\pr{}{x_t=x, a_t=a}.
\end{align*}

Since $P(x|x',a) = p(x)$, we simply have $\mu(x) := \mu(x,1) + \mu(x,0) = p(x)$ (by the first two constraints in LP \eqref{eq:CMDP-opt2} that characterize occupation measures). Notice that problem \eqref{eq:CMDP-opt2} is feasible by the assumption that $\forall x\in \candidateS, p(x) > 0$.

Let $\optmu$ be an optimal solution of the LP \eqref{eq:CMDP-opt2}. Then an optimal stationary policy for the CMDP \eqref{eq:CMDP-opt1} is given by: 
\begin{align*}
    \optpi(x,a) = \frac{\optmu(x,a)}{\sum_{a'} \optmu(x, a')} = \frac{\optmu(x,a)}{ p(x)}.
\end{align*}
 

\begin{lemma}\label{lem:constraint2target}
$g^\pi$ is the selection rate under policy $\pi$: $g^\pi = \langle \mu, r\rangle = \mathbb{P}^{p,\pi}[a=1].$
Moreover, if $\pi$ is feasible for CMDP \eqref{eq:CMDP-opt1}, then:  
\begin{align*}\forall i \in [d], \forall j \in \intint{\size_i}, \mathbb{P}^{p,\pi}[x_i=j | a=1] =\target_i^j.
\end{align*}
\end{lemma}

Lemma \ref{lem:constraint2target} states that (a) $\pi^*$ maximises the selection rate of candidates, and (b) the constraints of \eqref{eq:CMDP-opt1} force candidates $x$ with $x_i = v_i^j$ to be accepted in proportions given by $\target^j_i$. %\footnotetext{not stated for $j=\size_i$, because it is redundant with the fact that $\sum_{j \in \size_i}target^j_i = 1$.} 
Next we study how well those proportions are respected when we shift from infinite to finite-sized committee selection.

A detailed example can be found in Appendix \ref{appendix:cmdp}.

\subsection{Theoretical guarantees}

We analyze the strategy \statioalg (\textbf{C}onstrained \textbf{C}ommittee \textbf{C}onstruction) where at each timestep, the agent observes candidates $x_t \sim p$, decides to accept $x_t$ by playing $a_t \sim \optpi(.|x_t)$ and stops when $K$ candidates have been accepted.

First, we formally relate the gain $g^\pi$ that we optimize for in \eqref{eq:CMDP-opt1} to the quantity of interest $\mathbb{E}^{p,\pi}[\tau]$.
\begin{lemma}\label{lem:gain2time}
For any stationary policy $\pi$, $\mathbb{E}^{p,\pi}[\tau] = \frac{K}{g^\pi}$.
\end{lemma} 
Lemma \ref{lem:gain2time} is a direct consequence of the fact that $\tau + K$ follows a negative binomial distribution with parameters $K$ and $1-g^\pi$, which are respectively the number of successes and the probability of failure, i.e. of rejecting a candidate under $\pi$. Note that this is only true because in our case the transition structure of the MDP ensures constant gain. A quick sanity check shows that if the agent systematically accepts all candidates, i.e. $g^\pi = 1$, then $\mathbb{E}^{p,\pi}[\tau] = K$, and that maximizing $g^\pi$ is equivalent to minimizing $\mathbb{E}^{p,\pi}[\tau]$. 

%Then, 
We exhibit a bound on the representation loss of \statioalg which follows the optimal stationary policy $\optpi$ of CMDP \eqref{eq:CMDP-opt1}.  %incurred by  following the stationary policy from the average-reward CMDP approach. 
Let $\tilde{d} = \sum_{i=1}^d (D_i - 1)$. 
%Note that
(When all attributes are binary, $\tilde{d} = d$.)

\begin{proposition}\label{prop:hoeffding-loss}
Let $\pi^*$ be an optimal stationary policy for CMDP \eqref{eq:CMDP-opt1}. Let $\delta > 0$. Then, %$\mathbb{P}^\pi\left[\loss{C_\tau} \leq \sqrt{\frac{\log(\frac{2\tilde{d}}{\delta})}{2K}}\right] \geq 1 - \delta.$
\vspace{-1mm}
\begin{align*}
    \mathbb{P}^{p,\pi^*}\left[\loss{C_\tau} \leq \sqrt{\frac{\log(\frac{2\tilde{d}}{\delta})}{2K}}\right] \geq 1 - \delta.
\end{align*}
\vspace{-1mm}
\end{proposition}

All proofs of this section are available in Appendix \ref{sec:proof-cmdp}.

The upper bound on the representation loss of \statioalg decreases with the committee size in $\sqrt{1/K}$. This shows that the stationary policy $\optpi$ works well for larger committees, although it acts independently from previously accepted candidates. The intuition is that for larger committees, adding a candidate has less impact on the current representation vector. It was the opposite in Example \ref{ex:small-committee} where the goal was to recruit a very small committee of size $K=4.$

% \begin{algorithm}[t]
% \caption{\statioalg algorithm. \label{alg:statio}}
%  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%  \Input{optimal policy $\pi^*$ of \eqref{eq:CMDP-opt1}, committee size $K$}
%  \Output{committee $C_\tau$}
%  $t\gets 0$, $C_0 \gets \emptyset$\;
%  \While{$\card{C_t} < K$ }{
%     $t\gets t+1$, observe $x_t \sim p$ and play $a_t \sim \optpi(.|x_t)$ \;
%     \lIf{$a_t = 1$}{$C_t \gets C_t \cup \{x_t\}$}
%  }
% \Return{$C_t$}
% \end{algorithm}




==> sections/oldies/old_problem_def.tex <==

\section{Formal setting}\label{sec:model}

\subsection{Problem definition}
Let $\candidateS = \candidateS_1 \times ... \times \candidateS_d$ be the product space of $d$ finite domains, each of size $\size_i = \card{\candidateS_i}$, and where we identify $\candidateS_i$ with $\intint{\size_i}= \{1, ..., \size_i\}$. Each candidate is represented by a \emph{characteristic vector} $x \in \candidateS$ with $d$ \emph{features}. Let $x_i \in \candidateS_i$ denote the value of the $i$-th feature. For each $i \in \intint{d}$, we consider a \emph{target vector} $\target_i \in (0,1)^{\size_i}$ with $\sum_{j=1}^{\size_i}\target^j_i = 1.$

The goal 
%of the decision-maker 
is to select a \emph{committee} $C$ of $K$ candidates that matches the target vector as closely as possible. %while minimizing the number of candidates screened.
For some set $C$, let $\ratio(C) \in \prod_{i=1}^d[0,1]^{\size_i}$ be the \emph{representation profile} of $C$, where $\ratio_i^j(C) = \frac{\card{\{x \in C: x_i = j\}}}{\card{C}}$. We define the \emph{representation loss} as $\|\ratio(C) - \target\|_\infty = \max_{i \in \intint{d}, j \in \intint{\size_i}} \vert\ratio_i^j(C) - \target^j_i\vert$. We evaluate the quality of the representation of $C$ by the $\ell^\infty$ metric because it offers strong guarantees.
%(other choices may be interesting to consider as well). 


The candidate database is infinite and the horizon as well. At each timestep $t \geq 1$, the agent observes a candidate $x(t)$ drawn i.i.d.\ from a
stationary distribution $p$ over $\candidateS$, i.e. $x(t) \sim p$. The decision-maker must immediately decide between two actions: \emph{accept} or \emph{reject} the candidate, which we respectively denote as $a_t=1$ and $a_t=0$. Let $C_t = \{x(t'): t' \leq t, a_{t'} = 1\}$ denote the set of all accepted candidates at the end of step $t$. Let $N(t) = \card{C_{t-1}} = \sum_{t'=1}^{t-1}\indic{a_{t'} = 1}$. Let $N^j_i(t) = \sum_{t'=1}^{t-1}\indic{x_i(t') =j, a_{t'} = 1}$ be the number of accepted candidates $x$ such that $x_i = j$ before time $t$.

Let $\tau$ be the first time when $K$ candidates have been accepted. The process stops at $\tau$ and the agent outputs the final committee $C_\tau$. 

The agent must identify a ``representative'' committee in as 
``few rounds'' as possible. More precisely, the agent following a (possibly randomized) algorithm $\ALG$ must achieve a good trade-off between the \emph{representation loss} $\loss{C_\tau}$ and the \emph{sample complexity} $\mathbb{E}^{p, \ALG}[\tau]$. We consider two settings: whether the candidate distribution is \emph{known} or \emph{unknown}.

We assume that any feature vector can be observed, i.e., $p(x) > 0$ for all $x$. %\footnote{Note that the joint distribution $p(x)$ does not need to be represented explicitly and may be given to the agent in compact form (e.g., a Bayesian network).} 
%We also typically have: $(p^j_i)_{i,j} \neq (\rho_i^j)_{i,j}$.


\begin{remark}
In this model, we simply ignore non-volunteers, since the agent only needs to make decisions for volunteers, which from now on we call \emph{candidates}. The joint distribution of characteristic vectors in the population of candidates is $p$.
\end{remark}


\subsection{Greedy strategy}\label{sec:greedy}

We describe a first simple strategy. In \greedyalg, the agent greedily accepts any candidate as long as the number of people in the committee with $x_i = j$ does not exceed the quota $\ceil{\target^j_i K} + \tol K$  for any $i,j$, where $\tol > 0$ is some tolerance parameter for the representation quality. For precision, the pseudocode is included in Appendix \ref{app:greedy}, Alg~\ref{alg:greedyalg}.

\begin{remark}
The representation loss incurred by \greedyalg can be easily bounded as follows:
\begin{align*}
    \loss{C_\tau} \mathop{\leq}_{a.s.} \frac{1}{K} + \tol.
\end{align*}
\end{remark}

% Similar to greedy in online knapsack?


This method is simple to interpret and implement, and can even be used when the candidate distribution $p$ is unknown. However, in the following example, we see that \greedyalg may be inefficient because it requires interacting with an arbitrarily large number of candidates to recruit a full committee. %However, it is inefficient in practice because it necessitates high sample sizes to output a committee, and it is highly sensitive to the tolerance parameter $\tol$, as we will show in Section ~\ref{sec:expes}. 


% We now propose a constrained MDP-based approach that achieves better performance, yet being nonadaptive.
% \virginie{Can we get a lower bound on $\expe{}{\tau}$, for a convincing comparison? Or are experiments enough?}

\begin{table}[]
\centering
\begin{tabular}{|l|ll|}
\hline
gender \textbackslash{} age & S & J \\
\hline
M & $\nicefrac12-\epsilon'$ & $\nicefrac14$ \\
F & $\nicefrac14$ & $\epsilon'$\\
\hline
\end{tabular}
\caption{Example candidate distribution $p$ with 2 binary features.}
\label{tab:example-dist}
\end{table}

\begin{example}\label{ex:small-committee}
Let $\epsilon' >0, \ll 1$. There are 2 binary features, \emph{gender} and \emph{age}, with domains $\candidateS_{\text{gender}}=\{M,F\}$ 
%(male, female) 
and $\candidateS_{\text{age}}=\{S,J\}$.
%(senior, junior). 
The candidates are distributed as $p$ given in Table \ref{tab:example-dist}. We want a committee of size $K = 4$ (e.g., a thesis committee) and the target is $\target_{\text{gender}}=(\nicefrac{1}{2}, \nicefrac{1}{2})$ and $\target_{\text{age}} = (\nicefrac{3}{4}, \nicefrac{1}{4})$.

Let $A$ be the event that in the first $3$ timesteps, the agent observes candidates with characteristic vectors $\{FS, MS, MS\}$ in any order. Then \greedyalg accepts all of them, i.e. $A = \left\{C_3 = \{FS, MS, MS\}\right\}$. We have: $\pr{}{A} = \nicefrac{1}{4} (\nicefrac{1}{2} - \epsilon')^2\times 3!  = \nicefrac{3}{2} (\nicefrac{1}{2} - \epsilon')^2 \geq \nicefrac{3}{2} \big(\nicefrac{1}{3}\big)^2 = \nicefrac16$.
%\begin{align*}
%    \pr{}{A} = \frac{1}{4} (\frac{1}{2} - \epsilon')^2\times 3! = \frac{3}{2} (\frac{1}{2} - \epsilon')^2 \geq \frac{3}{2} \big(\frac{1}{3}\big)^2 = \frac{1}{6}
%\end{align*}

Under event $A$, \greedyalg can only stop upon finding $FJ$ in order to satisfy the representation constraints. Therefore, $\tau | A$ follows a geometric distribution with success probability $\epsilon'$, hence its expectation is $\nicefrac{1}{\epsilon'}$, and
%\begin{align*}
%    \mathbb{E}^{p,\greedyalg}[\tau] \geq \expe{}{\tau|A}\times\pr{}{A} = \frac{1}{6\epsilon'}.
%\end{align*}
$\mathbb{E}^{p,\greedyalg}[\tau] \geq \expe{}{\tau|A}\times\pr{}{A} = \nicefrac{1}{6\epsilon'}.$
Therefore, the sample complexity of \greedyalg in this example is arbitrarily large. 
%To avoid the obstacle of event $A$,  a good strategy should reject one $MS$ and accept one $FS$ instead. Indeed, having accepted $C_t = \{FS,MS,FS\}$, it will stop with a perfectly representative committee as soon as one $MJ$ arrives.
%(which occurs with probability $\nicefrac{1}{4} \gg \epsilon'$).
\end{example}

This example shows the limits of directly applying a naive strategy to our online selection problem, where the difficulty arises from considering multiple features simultaneously, even when there are only $2$ binary features. We further discuss the strengths and weaknesses of \greedyalg, and its sensitivity to the tolerance $\tol$ in our experiments in Section \ref{sec:expes}.

The greedy strategy is adaptive, in the sense that decisions are made based on the current candidate and candidates accepted in the past. In the following section, we present, with theoretical guarantees, an efficient yet non-adaptive algorithm based on constrained MDPs for the setting in which the candidate distribution is known. We then adapt this approach to the case when this distribution is unknown, using techniques for efficient exploration / exploitation in constrained MDPs relying on the principle of optimism in the face of uncertainty.

% In the following sections, we present a strategy based on constrained MDPs with provable guarantees when the candidate distribution is known. We adapt this approach to the case when this distribution is unknown, using techniques for exploration / exploitation in constrained MDPs based on the principle of optimism in the face of uncertainty.

%and show how the latter, although non-adaptive, achieves better trade-offs than the greedy adaptive policy.

%In  the  following  sections,  we  present  two  strategies  V:now it is three settings, a greedy adaptive policy and a con-strained MDP-based stationary policy, and show how the latter, although non-adaptive, achieves better trade-offs than the greedy adaptive policy.

==> sections/oldies/old_proofs.tex <==
\section{Proofs}\label{sec:proofs}

\subsection{Proofs of Section \ref{sec:cmdp}}\label{sec:proof-cmdp}

Proof of Lemma \ref{lem:constraint2target}.

\begin{proof}
\begin{align*}
    g^\pi &= \sum_{x,a} \mu(x,a) r(x,a) = \sum_{x} \mu(x) \sum_a \pi(x,a) r(x,a)\\
    &= \expe{\substack{x \sim p\\ a \sim \pi(.|x)}}{r(x,a)} = \mathbb{P}^\pi[a=1].
\end{align*}
The first equality is by definition of the occupation measure, and the third equality is by the observation $\mu(x) = p(x)$ for all $x \in \candidateS$.

Next, we observe that:
\begin{align*}
\langle\mu, r^j_i\rangle &= \sum_{x, a} \mu(x) \pi(x,a) r^j_i(x,a) = \expe{\substack{x \sim p \\ a \sim \pi(\cdot|x)}}{r^j_i(x,a)} \\
&= \mathbb{P}^{p, \pi}[a=1, x_i=j],\\
\end{align*} 
\begin{align*}
    \text{and }\quad\frac{\langle\mu, r^j_i\rangle}{\langle\mu, r\rangle} =\frac{\mathbb{P}^{p,\pi}[a=1, x_i=j]}{\mathbb{P}^{p,\pi}[a=1]} = \mathbb{P}[x_i=j|a=1].
\end{align*} By the last constraint of \eqref{eq:CMDP-opt2}, we have, for all $i \in [d]$ and $j \in \intint{\size_i-1}$, $\frac{\langle\mu, r^j_i\rangle}{\langle\mu, r\rangle} = \target^j_i$, which gives the result. Note that the results also holds true for $j = \intint{\size_i}$, since \begin{align*}
&\mathbb{P}[x_i=\size_i|a=1] = 1 - \sum_{j' \in \intint{\size_i - 1}} \mathbb{P}[x_i=j'|a=1] &\text{ and } \\ &\target^{\size_i}_i = 1 - \sum_{j' \in \intint{\size_i - 1}} \target^{j'}_i. 
\end{align*}

\end{proof}


Proof of Proposition \ref{prop:hoeffding-loss}.

\begin{proof} 
For any $t > 0$, we have $$\ratio^j_i(C_t) = \frac{N^j_i(t)}{N(t)} = \frac{\sum_{s=1}^t \indic{x_i(s)=j, a_s=1}}{\sum_{s=1}^t \indic{a_s=1}}.$$

and by Lemma \ref{lem:constraint2target}, we have: $$\expe{}{\indic{x_i=j} \vert a = 1} = \target^j_i.$$

% Since all draws of $x_i^j(s)$ are independent, by Hoeffding's inequality \cite{hoeffding1994probability}, we have for any %$\alpha > 0$, $\pr{}{|\ratio^j_i(C_t) - \target^j_i| \geq \alpha } \leq e^{-2t\alpha^2}$. 
% $\delta' > 0$,  $\pr{}{|\ratio^j_i(C_t) - \target^j_i| \leq \sqrt{\frac{\log(\frac{2}{\delta'})}{ N(t)}} }\geq 1 - \delta'$. 

% Let $\delta' >0$.

% \begin{align*}
%     &\pr{}{|\ratio^j_i(C_\tau) - \target^j_i| \geq \sqrt{\frac{\log(\frac{\pi^2K^2}{3\delta'})}{2 K}}} \\
%     &= \pr{}{|\ratio^j_i(C_\tau) - \target^j_i| \geq \sqrt{\frac{\log(\frac{\pi^2N(\tau)^2}{3\delta'})}{2 N(\tau)}}}\\
%     &\leq \pr{}{\bigcup_{t = 1}^{\infty}|\ratio^j_i(C_t) - \target^j_i| \geq \sqrt{\frac{\log(\frac{\pi^2N(t)^2}{3\delta'})}{2 N(t)}}} \\
%     &\leq \sum_{t = 1}^{\infty}\pr{}{|\ratio^j_i(C_t) - \target^j_i| \geq \sqrt{\frac{\log(\frac{\pi^2N(t)^2}{3\delta'})}{2 N(t)}}} \\
%     &\leq \sum_{t = 1}^{\infty} 2 \times \frac{3 \delta'}{\pi^2 N(t)^2} \leq \delta'\, 
% \end{align*}

% where the first equality is because $N(\tau) = K$, by definition of $\tau$, and the penultimate inequality by Hoeffding's inequality.

% The result follows from applying a union bound over all $i \in \intint{d}, j \in \intint{D_i - 1}$ (there are $\tilde{d}$ such $(i,j)$ pairs) and choosing $\delta' = \delta / \tilde{d}$. 

Let $\delta'>0$. Conditionally on any $T \geq K, (a_1, ..., a_T) \in \{0,1\}^T$ s.t. $a_1+ ...+a_T=K$ and $a_T=1$, the draws of $x_i(t)|a_t=1$ are independent and thus, by Hoeffding's inequality \cite{hoeffding1994probability}, we have:

\begin{align*}
&\pr{}{|\ratio^j_i(C_T) - \target^j_i| \geq \sqrt{\frac{\log(\frac{2}{\delta'})}{2 N(T)}}\bigg\vert a_1, ..., a_T} \geq 1- \delta'\\
&=\pr{}{|\ratio^j_i(C_T) - \target^j_i| \geq \sqrt{\frac{\log(\frac{2}{\delta'})}{2 K}}\bigg\vert a_1, ..., a_T}.
\end{align*}

Summing up over all such sequences $(a_1,..., a_T)$, we obtain that: 
\begin{align*}
&\pr{}{|\ratio^j_i(C_\tau) - \target^j_i| \geq \sqrt{\frac{\log(\frac{2}{\delta'})}{2 K}}} \geq 1- \delta'.
\end{align*}
The result follows from applying a union bound over all $i \in \intint{d}, j \in \intint{D_i - 1}$ (there are $\tilde{d}$ such $(i,j)$ pairs) and choosing $\delta' = \delta / \tilde{d}$.

% \virginie{
% We define the filtration $\mathcal{F}_t = \sigma(x_1, a_1, ..., x_{t+1})$. Recall that $\tau = \inf(\{t \geq 0:  N(t) \geq K\})$. Let $k_s$ be the time when action $1$ was played for the $s$-th time. Both $\tau$ and $k_s$ are stopping times w.r.t. $(\mathcal{F}_s)_s$. We have: 
% \begin{align*}
%     &N^j_i(\tau) = \sum_{s=1}^{\tau} \indic{x^j_i(s), a_s = 1} = \sum_{s=1}^{K} \indic{x^j_i(k_s) = 1} &\text{ and }\\
%     &N(\tau) = \sum_{s=1}^\tau \indic{a_s = 1} = \sum_{s=1}^{K} 1 = K. 
% \end{align*}

% Let $M_t = \indic{x^j_i(k_t) = 1} - \target_i^j$.

% \begin{align*}
%     \expe{}{\indic{x^j_i(k_s) = 1} | \filtr_{s-1}} & = \sum_{k > 0}\indic{k_s = k} \expe{}{\indic{x^j_i(k) = 1} | \filtr_{s-1}}\\
%     & = \mathbb{E}[\indic{x^j_i=1}|a=1] = \target^j_i.
% \end{align*}
% where the last equality is by Lemma \ref{lem:constraint2target}.

% Therefore, $(M_s)_s$ is a martingale difference sequence. By Azuma-Hoeffding's inequality, for all $\delta' > 0$, we have:

% \begin{align*}
%   \pr{}{\sum_{s=1}^K \left(\indic{x^j_i(s)} - \target_i^j \right) \geq \sqrt{2K\log(\frac{2}{\delta'})}} \leq \delta'
% \end{align*}


% }

% {\color{red}
% I think it is much simpler than this.

% Here a very quick and sketched proof.
% Let $x(t) \sim p$ and $a(t) \sim \pi(x_t)$.
% Define the filtration $\mathcal{F}_t$ to include all the history up to time $t$, $x(t)$ included.
% Let $B_k = \sum_{t=1}^k 1(a(t) = 1)$ and $\tau = \inf(\{k \geq 0:  B_k > K\})$, $K >0$ fixed in advance.

% Let
% $N^j(\tau) = \sum_{s=1}^\tau 1(x^j(s) = i) 1(a(s) = 1) = \sum_{s=1}^{K} 1(x^j(k_s) = 1)$ and
% $N(t) = \sum_{s=1}^\tau 1(a(s) = 1) = \sum_{s=1}^{K} 1 = K$
% with $k_s$ being the the s-th time action $1$ was played.
% Both $\tau$ and $k_s$ are stopping times wrt $(\mathcal{F}_s)_s$. 


% Now we have that $(1(x^j(k_s) = 1) - \rho_i^j)_s$ is an MDS (check!) wrt the filtrations $(\mathcal{F}_s)$.
% Then by using Azuma-Hoeffding we have that
% \[
%   \forall j, \mathbb{P}\left( \sum_{s=1}^K \left(1(x^j(k_s) = 1) - \rho_i \right) \geq \sqrt{2K \ln(1/\delta)} \right) \leq \delta
% \]
% }

\end{proof}

\subsection{Proof of Theorem \ref{thm:regret}}\label{sec:proof-regret}

% The following lemma can be found in Auer or Weissman \virginie{or use bernstein or whatever does the job.}
% \begin{lemma}\label{lem:probainterval} Let $\delta > 0$ and $B_l = \{\tilde{p} \in \Delta(\candidateS): \|\hat{p}_\iepi - \tilde{p}\|_{1} \leq  \rad_\iepi\}$. Then,
% \begin{align*}
%   \pr{}{\exists \iepi \geq 1, \prepi \notin B_\iepi} \leq \delta / 3 
% \end{align*}
% \end{lemma}

% The following lemma states two useful and standard inequalities, see. e.g., Lem. 13 in \cite{pmlr-v97-zanette19a} for the first and Lem. 19 in \cite{jaksch2010near} for the second.
% \begin{lemma}\label{lem:sum-integrals} Recall that $\nepi$ is the random number of episodes ran by \optalg up until horizon $T$. We have:
% \begin{align*}
%     \sum_{\iepi=1}^{\nepi} \frac{\durepi}{\tepi_\iepi -1} \leq \log(T) &\quad \text{and} & \sum_{\iepi=1}^{\nepi} \frac{\durepi}{\sqrt{\tepi_\iepi}} \leq 2 \sqrt{T}
% \end{align*}
% \end{lemma}

The following lemma states a standard and useful inequality, which is similar to Lem. 19 in \cite{jaksch2010near}.
\begin{lemma}\label{lem:sum-integrals} Recall that $\nepi$ is the random number of episodes ran by \optalg up until horizon $T$. We have:
\begin{align*}
    \sum_{\iepi=1}^{\nepi} \frac{\card{\durepi}}{\sqrt{\tepi_\iepi - 1}} \leq 2 \sqrt{T}.
\end{align*}
\end{lemma}

\begin{proof}
The proof is similar to that of Lem. 13 in \cite{zanette2019tighter}: we see $\durepi$ as the ``derivative'' of ${\tepi_\iepi}$. Formally, let us define:
\begin{align*}
    &F(x) = \sum_{\iepi=1}^{\floor{x}}\card{\durepi} + \card{E_{\ceil{x}}}(x - \floor{x}) \\
    &f(x) := F'(x) = \card{E_{\ceil{x}}}.
\end{align*}
We first observe that for any integer $\iepi \in \mathbb{N}$, $f(\iepi) = \card{\durepi}$ and $F(\iepi) = \tepi_\iepi.$ Secondly, we have \begin{align*}
     F(x) \leq \sum_{\iepi=1}^{\floor{x}}\card{\durepi} + \card{E_{\ceil{x}}} = \sum_{\iepi=1}^{\ceil{x}}\card{\durepi} = F(\ceil{x}),
\end{align*} and thus:
$$\frac{f(\ceil{x})}{\sqrt{F(\ceil{x})-1}}  \\
    \leq\frac{f(x)}{\sqrt{F(x)-1}}.$$

We derive our bound as follows:
\begin{align*}
    \sum_{\iepi=1}^{\nepi} \frac{\card{\durepi}}{\sqrt{\tepi_\iepi - 1}} &= \sum_{\iepi=1}^{\nepi} \frac{f(\iepi)}{\sqrt{F(\iepi) - 1}} =  \int_{1}^{\nepi}\frac{f(\ceil{x})}{\sqrt{F(\ceil{x})-1}} \,dx \\
    &\leq \int_{1}^{\nepi}\frac{f(x)}{\sqrt{F(x)-1}} \,dx = 2(\sqrt{F(\nepi) - 1}) \\
   & = 2(\sqrt{\tepi_\nepi - 1}) \leq 2 \sqrt{T}.
\end{align*}

\end{proof}

We introduce the following notation: for $f:\candidateS \times \actS \rightarrow \mathbb{R}$, let $f^\pi(x) := \sum_{a} f(x, a) \pi(x,a)$. For all $t > 0$, let $\iepi_t$ denote the episode number at time $t$. The following useful lemma is based on a martingale argument.
\begin{lemma}\label{lem:azuma} Let $f:\candidateS \times \actS \rightarrow \mathbb{R}$. Let $\delta' > 0$. We have:
% \begin{align*}
%     \pr{}{\sum_{t=1}^T(\langle r^{\piepit}, p\rangle - r(x_t, a_t)) \leq \sqrt{T \log(1/\delta')}} \geq 1 - \delta'\\
%     \pr{}{\sum_{t=1}^T(\langle {\cstr_j^i}^{\piepit}, p\rangle - {\cstr_j^i}(x_t, a_t)) \leq \sqrt{T \log(1/\delta')}} \geq 1 - \delta'\\
% \end{align*}
\begin{align*}
    \pr{}{\sum_{t=1}^T(\langle f^{\piepit}, p\rangle - f(x_t, a_t)) \leq \sqrt{2T \log(1/\delta')}} \geq 1 - \delta'\\
    \pr{}{\sum_{t=1}^T\big\vert\langle f^{\piepit}, p\rangle - f(x_t, a_t)\big\vert \leq \sqrt{2T \log(2/\delta')}} \geq 1 - \delta'.
\end{align*}
\end{lemma}

\begin{proof}
We define the filtration $\filtr_{t} = \sigma(x_1, a_1, ..., x_t, a_t)$ and we first show that the sequence defined by $M_t = \langle f^{\piepit}, p\rangle - f(x_t, a_t)$ is a martingale difference sequence w.r.t. $\filtr_{t}$. $\expe{}{M_t} < \infty$ since the rewards are bounded. Next, the proof that $\expe{}{M_t|\filtr_{t-1}} = 0$ relies on the fact that $\iepi_t$, and in turn the stationary policy $\piepit$, are $\filtr_{t-1}-$measurable.
% \begin{align*}
%     \expe{}{\langle r^{\piepit}, p\rangle \big| \filtr_{t-1}} =\sum_{x,a} r(x,a) p(x)  \expe{}{\piepit(x,a) \big\vert \filtr_{t-1}}
% \end{align*}

% \begin{align*}
%     \expe{}{r(x_t, a_t) \big| \filtr_{t-1}} = \expe{}{\sum_{x,a} r(x,a) \indic{(x_t, a_t) = (x,a)} \bigg\vert \filtr_{t-1}}\\
%     = \sum_{x,a} r(x,a)  \sum_{\iepi}\expe{}{\indic{(x_t, a_t) = (x,a)}\indic{\iepi_t = \iepi}  \big\vert \filtr_{t-1}} \\
%     = \sum_{x,a} r(x,a) \sum_{\iepi}\indic{\iepi_t = \iepi} \expe{}{\indic{(x_t, a_t) = (x,a)} \big\vert \filtr_{t-1}} \\
%     % = \sum_{x,a} r(x,a) \sum_{\iepi}\indic{\iepi_t = \iepi} \expe{}{\indic{(x_t, a_t) = (x,a)}} \\
%     = \sum_{x,a} r(x,a) \sum_{\iepi}\indic{\iepi_t = \iepi} p(x)\piepi(x,a)\\
%     = \sum_{x,a} r(x,a) p(x) \expe{}{\piepit(x,a)\big\vert \filtr_{t-1}} \\
% \end{align*}
% The third and last equality are by $\filtr_{t-1}-$measurability, and the fourth equality is because $(x_t, a_t)$ is independent of $\filtr_{t-1}$ and when $\iepi_t = l$, $\pr{}{(x_t, a_t) = (x,a)} = p(x)\piepi(x,a)$. Subtracting the two expressions above, we get $\expe{}{M_t|\filtr_{t-1}} = 0$. 

Therefore, 
\begin{align*}
    \expe{}{\langle f^{\piepit}, p\rangle \big| \filtr_{t-1}} = \langle f^{\piepit}, p\rangle. 
\end{align*}

We also have: 

\begin{align*}
    \expe{}{f(x_t, a_t) \big| \filtr_{t-1}} &= \expe{}{\sum_{x,a} f(x,a) \indic{(x_t, a_t) = (x,a)} \bigg\vert \filtr_{t-1}}\\
    &= \sum_{x,a} f(x,a) \piepit(x,a) = \langle f^{\piepit}, p\rangle.
\end{align*}

Subtracting the two expressions above, we get $\expe{}{M_t|\filtr_{t-1}} = 0$. $(M_t)_{t}$ is thus a Martingale difference sequence, such that $-1\leq M_t \leq 1$. The result follows from Azuma-Hoeffding's inequality.

\end{proof}

We now prove Theorem~\ref{thm:regret}.

\begin{proof} 
We define $\mathcal{E} = \mathcal{E}_1 \cap\mathcal{E}_2  \cap\mathcal{E}_3 $ to be the ``good event'', with:
\begin{align*}
    &\mathcal{E}_1 = \{\forall \iepi \geq 1, \prepi \in B_\iepi\},\\
    &\mathcal{E}_2 = \{\sum_{t=1}^T(\langle r^{\piepit}, p\rangle - r(x_t, a_t)) \leq \sqrt{2T \log(3/\delta)}\}, \\
    &\mathcal{E}_3 = \left\{\forall i,j, \quad \sum_{t=1}^T\big\vert\langle {\cstr^j_i}^{\piepit}, p\rangle - {\cstr^j_i}(x_t, a_t)\big\vert \leq \sqrt{2T \log\big(\frac{6\tilde{d}}{\delta}\big)}\right\}.
\end{align*}

By Lemma \ref{lem:l1-dev}, we have
\begin{align}\label{eq:probinterval}
    \pr{}{\exists \iepi \geq 1, \prepi \in B_\iepi} \geq 1- \frac{\delta}{3}. 
\end{align}
Combining \eqref{eq:probinterval} with Lemma \ref{lem:azuma} and using union bounds, $\pr{}{\mathcal{E}} \geq 1 - \delta$. From now on, we assume that the good event $\mathcal{E}$ holds true.

\paragraph{Performance regret} We start by upper bounding the performance regret $\regret(T)$. Let $\Delta_\iepi = \sumepi (g^* - r(x_t, a_t))$ be the regret of episode $\iepi$. Let $(\pi_\iepi, \tilde{p}_\iepi)$ be the solution of the optimistic CMDP \eqref{eq:OptCMDP-1} at episode $\iepi$. Since $(\pi^*, p)$ is feasible for \eqref{eq:OptCMDP-1}, then $g^* \leq g^{\prepi,\piepi}$. We also note that $$g^{\prepi,\piepi} = \sum_{x,a} r(x,a)\prepi(x)\piepi(x,a) = \sum_{x} r^{\piepi}(x)\prepi(x),$$
since $\mu(x) = \tilde{p}_l(x)$ and $\mu(x,a) = \mu(x)\pi_l(x,a)$.
Therefore, we have:
\begin{equation}\label{eq:bound-epi-reg}
\begin{aligned}
    \Delta_\iepi &\leq \sumepi (g^{\prepi,\piepi} - r(x_t, a_t))\\
    &= \sumepi (\sum_{x} r^{\piepi}(x)\prepi(x) - r(x_t, a_t))\\
    &= \sumepi \sum_{x} r^{\piepi}(x)(\prepi(x) - p(x))\\
    & \quad + \sumepi(\sum_{x} r^{\piepi}(x)p(x) - r(x_t, a_t))\,
\end{aligned}
\end{equation}



Using Hölder's inequality and the fact that $\|r\|_{\infty} = 1$, the first term can be bounded by $\card{\durepi} \|\prepi - p\|_{1}$. By validity of the confidence intervals under event $\mathcal{E}$:
\begin{equation}
\begin{aligned}
    \|\prepi - p\|_{1} \leq 2 \radepi \leq \frac{2 \sqrt{2\ncand\log\big(6\ncand T (T-1) / \delta\big)}}{\sqrt{\tepi_\iepi -1}}
\end{aligned}
\end{equation}

Summing up over episodes $\iepi=1,..., \nepi$:
\begin{equation}
\begin{aligned}
    \regret(T) &\leq 2 \sqrt{2\ncand\log\big(\frac{6\ncand T (T-1)}{ \delta}\big)}\sum_{\iepi=1}^{\nepi}\frac{\card{\durepi} }{\sqrt{\tepi_\iepi -1}} \\
    &+ \sum_{t=1}^T(\sum_{x} r^{\piepit}(x)p(x) - r(x_t, a_t)).
\end{aligned} 
\end{equation}


We bound the first sum using Lemma \ref{lem:sum-integrals}. The second term can be bounded as in Lemma \ref{lem:azuma} because $\mathcal{E}_2$ holds true. This gives us the resulting bound which holds under $\mathcal{E}$:
\begin{equation*}
\begin{aligned}
    \regret(T) &\leq 4 \sqrt{\ncand\log\big(\frac{6\ncand T (T-1)}{ \delta}\big)T} + \sqrt{2T \log\big(\frac{3}{\delta}\big)}.
\end{aligned} 
\end{equation*}


\paragraph{Cost of constraint violations} The proof for the cost of constraint violations is very similar. Let us bound $\regret_i^j(T) := \sum_{t=1}^T |\cstr_i^j(x_t, a_t)|$ for all $i,j$. We briefly drop the sub/superscripts $i,j$.

At each episode $\iepi$, since $(\piepi, \prepi)$ is a solution of \eqref{eq:OptCMDP-1}, we have $h^{\prepi, \piepi}=0$, and thus $\sum_{x,a}\cstr(x,a)\piepi(x,a)\prepi(x) = \sum_{x}\cstr^{\piepi}(x)\prepi(x) = 0$. Therefore, we have:

\begin{align*}
    \abs{\sum_{t=1}^T \cstr(x_t, a_t)} &= \abs{\sum_{\iepi=1}^{\nepi}\big(\sumepi \cstr(x_t, a_t) - \sum_{x} \cstr^{\piepi} (x)\prepi(x)\big)} \\ &\leq\bigg\vert \sum_{\iepi=1}^{\nepi}\sumepi\sum_{x} \cstr^{\piepi} (x)(p(x) - \prepi(x))\\
    & \quad \quad + \sum_{\iepi=1}^{\nepi}\big(\sumepi\cstr(x_t, a_t) - \sum_{x} \cstr^{\piepi}(x)p(x) \big)\bigg\vert\\
    &\leq \sum_{\iepi=1}^{\nepi}\sumepi\abs{\sum_{x} \cstr^{\piepi} (x)(p(x) - \prepi(x))}\\
    & \quad \quad + \abs{\sum_{\iepi=1}^{\nepi}\big(\sumepi\cstr(x_t, a_t) - \sum_{x} \cstr^{\piepi}(x)p(x) \big)}\\
    &\leq \sum_{\iepi=1}^{\nepi}\card{\durepi}\|\cstr^{\piepi}\|_{\infty}\|p - \prepi\|_1\\
    & \quad \quad + \abs{\sum_{t=1}^T \bigg(\cstr(x_t, a_t) - \sum_{x} \cstr^{\piepit}(x)p(x)\bigg)},\\
\end{align*}
where the first part of the last inequality is again by Hölder's inequality. Similarly to the performance regret,  the first term is bounded using the validity of confidence intervals under the good event $\mathcal{E}$ and Lemma \ref{lem:sum-integrals}, and the second term is bounded by the martingale argument using Lemma \ref{lem:azuma}. Hence, under $\mathcal{E}$ we have for any $i,j$:
\begin{equation*}
\begin{aligned}
    R^j_i(T) &\leq 4 \sqrt{\ncand\log\big(\frac{6\ncand T (T-1)}{ \delta}\big)T} + \sqrt{2T \log\big(\frac{6\tilde{d}}{\delta}\big)}.
\end{aligned} 
\end{equation*}

And thus the same bounds holds for $\violate(T) = \max_{i,j} R^j_i(T)$.

\paragraph{Representation loss}
We may now derive the bound on representation loss.

Let $f(T) = O\big(\sqrt{\ncand \log(\ncand T/\delta)}\big)$. The regret bounds imply that with $1- \delta$:
\begin{align*}
    R(T) &= g^*T - N(T) \leq f(T)\\
    \frac{R^c(T)}{N(T)} &= \max_{i,j} \abs{\frac{N^j_i(T)}{N(T)} - \target^j_i \frac{N(T)}{N(T)}}\leq \frac{f(T)}{N(T)}\\
    &= \|\ratio(C_T) - \target\|_{\infty}.
\end{align*}
Therefore, we have: 
\begin{align*}
    \|\ratio(C_T) - \target\|_{\infty}\leq \frac{f(T)}{g^*T - f(T)} = O\bigg(\sqrt{\frac{\ncand \log(\ncand T/\delta)}{{g^*}^2T}}\bigg).
\end{align*}
\end{proof}





==> sections/oldies/older_mdp.tex <==
\section{Constrained MDP approach} \label{sec:cmdp}\virginie{name of the section?}

In this approach, we place ourselves in the limit where we would select a committee of infinite size, and aim to maximise the rate at which candidates are selected, under the constraint that the proportion of accepted candidates per feature value is controlled by $\target$. One advantage of this approximation is that the optimal policy is stationary, thus simple to represent. Moreover, stationary policies can be very well parallelized, in the case where multiple candidates are interviewed simultaneously. To apply this approach to the finite-size committee selection problem, one needs to interrupt the agent when $K$ candidates have been selected. We showcase a high probability bound of $O(\sqrt{1/K})$ on the representation loss, which guarantees that for large enough values of $K$, the resulting committee is representative. 

%\virginie{Stationary policies are very simple to calculate and implement, even if parallelism. Non adaptive, but it's not so much of problem, which is what we show. (-- conclusion : in future work, we do adaptive)}

\subsection{Background} 
An MDP is a tuple $(\stateS, \actS, P, r)$, where $\stateS$ is the set of states, $\actS$ is the set of actions, $P:\stateS \times \actS \times \stateS \rightarrow [0, 1]$ is the transition kernel such that $P(x'|x, a)$ is the probability to be in state $x'$ given that the previous state was $x$ and the agent took action $a$, and $r:\stateS\times \actS \rightarrow \mathbb{R}$ is the mean of the reward distribution. We consider the \emph{average reward} setting in which the performance of a policy $\pi:\stateS \times \actS \rightarrow [0, 1]$ is measured by its \emph{gain} $g^{P,\pi}$, defined as:
\begin{align*}
g^{P,\pi}(x) = \lim_{T \rightarrow \infty} \frac{1}{T} \mathbb{E}^{P,\pi}\left[\sum_{t=1}^T r(x_t, a_t) \bigg\vert x_1 = x\right].
\end{align*}
We simply write $g^{P,\pi} := g^{\pi}$ when the underlying transition is $P$ without ambiguity.

A constrained MDP (CMDP) \cite{altman1999constrained} is an MDP where the set of allowed policies is restricted by a set of additional $\nconstraints$ constraints, specified by reward distributions with means $\cstr_k: \stateS \times \actS \rightarrow [0, 1]$ and constant bounds $b_k$ for $k \in \intint{m}$. Similarly to the gain, we define $h_k^\pi = \lim_{T \rightarrow \infty} \frac{1}{T} \mathbb{E}^\pi\left[\sum_{t=1}^T \cstr_k(x_t, a_t)\right]$. The CMDP is defined by:
\begin{align}\label{eq:CMDP-opt1}
    \max_{\pi} \{g^\pi | \forall k \in \intint{\nconstraints}, h_k^\pi \leq b_k \}
\end{align}
For unichain MDPs, the gain is constant, i.e. $\forall x \in \stateS, g^\pi(x) = g^\pi$, and the problem \eqref{eq:CMDP-opt1} is well defined. Then the CMDP can be solved by solving the equivalent linear program (LP) \cite{altman1999constrained}: 
\begin{equation}\label{eq:CMDP-opt2}
\begin{aligned}
\max_{\mu \in \reals^{\candidateS \times \actS}} \quad & \langle \mu, r \rangle  \\
\text{u.c.} \quad & \mu \geq 0, \sum_{x,a} \mu(x,a)  = 1 \\
& \forall x' \in \stateS, \sum_{x}\sum_{a} \mu(x,a) P(x'|x, a) = \sum_{a}\mu(x', a) \\
& \forall k \in [\nconstraints], \langle\mu, \cstr_k \rangle \leq b_k. \\
\end{aligned}
\end{equation}

$\mu : {\candidateS \times \actS} \rightarrow [0, 1]$ is said to be an \emph{occupation measure} \cite{altman1999constrained}, and is defined as: 
\begin{align*}
    \mu(x,a) = \lim_{T\rightarrow \infty}\frac{1}{T}\sum_{t=1}^T\pr{}{x_t=x, a_t=a}.
\end{align*}

Let $\optmu$ be an optimal solution of the LP \eqref{eq:CMDP-opt2}. Then an optimal stationary policy for the CMDP \eqref{eq:CMDP-opt1} is given by: $\optpi(x,a) = \optmu(x,a) / \sum_{a'} \optmu(x, a')$.

\subsection{Our model}\label{sec:cmdp-ourmodel}
We now formalize our committee selection problem as a very simple constrained MDP in which actions do not impact the next state. Fundamentally, our problem can be seen as a contextual bandit with stochastic contexts $x_t \sim p$ and two actions $a = 0$ or $1$. However, the type of constraints incurred by proportional representation are well studied in CMDPs, whereas the contextual bandits literature focused on other constraints (e.g., knapsack constraints \cite{agrawal2016linear}).

Formally, in our setting, the state space is the $d$-dimensional candidate space $\stateS := \candidateS$ and the set of actions is simply $\actS = \{0, 1\}$. First notice that $P(x'|x,a) =  p(x')$ since the candidates are drawn i.i.d.\ regardless of the previous actions and observed candidates, and subsequently we simply have $\mu(x) := \mu(x,1) + \mu(x,0) = p(x)$ (by the first two constraints in LP \eqref{eq:CMDP-opt2} that characterize occupation measures). Importantly, given the simplicity of the transition kernel, the gain is \emph{constant}, i.e. it does not depend on the start state. {\color{purple} [M:More, the MDP is ergodic since $p(x) > 0$]} From now on, we only write $g^\pi$ and $\cstr^\pi$.

%\footnotetext{Note that since $p > 0$, the MDP is \emph{communicating} \cite{puterman2014markov}, which ensures constant gain of any optimal policy. This is not as important in our case since the transition does not depend on the previous state.} 

We define the reward to be $r(x,a) = \indic{a=1}$. In order to fit the classical CMDP framework, we also need to define a reward for each constraint. We introduce $r_i^j$ as $r_i^j(x, a) = \indic{x_i^j=1, a=1}$. Then, let $\cstr_i^j = r_i^j - \target_i^j r$. The optimal stationary policy is $\optpi(x,a) = \frac{\optmu(x,a)}{\optmu(x,1) + \optmu(x,0)}$, where $\optmu$ is the optimal solution of the LP \eqref{eq:CMDP-opt2}, in which the constraints on the last line can be re-written as: 
\begin{align} \label{eq:CMDP-opt3}
  \forall i \in [d], \forall j \in \intint{\size_i - 1}, \langle\mu, \cstr^j_i\rangle = 0.
\end{align}

Problem \eqref{eq:CMDP-opt2} with constraints \eqref{eq:CMDP-opt3} is feasible by the assumption that $\forall x\in \candidateS, p(x) > 0$.
\begin{lemma}\label{lem:constraint2target}
$g^\pi$ is the selection rate under policy $\pi$: $g^\pi = \langle \mu, r\rangle = \mathbb{P}^{p,\pi}[a=1].$
Moreover, if $\pi$ is feasible for CMDP \eqref{eq:CMDP-opt1}, then:  
\begin{align*}\forall i \in [d], \forall j \in \intint{\size_i}, \mathbb{P}^{p,\pi}[x^j_i=1 | a=1] =\target_i^j.
\end{align*}
\end{lemma}

Lemma \ref{lem:constraint2target} states that (a) $\pi^*$ maximises the selection rate of candidates, and (b) the constraints \eqref{eq:CMDP-opt3} force candidates $x$ with $x_i = v_i^j$ to be accepted in proportions given by $\target^j_i$. %\footnotetext{not stated for $j=\size_i$, because it is redundant with the fact that $\sum_{j \in \size_i}target^j_i = 1$.} 
Next we study how well those proportions are respected when we move away from the infinite committee selection setting by stopping as soon as $K$ candidates have been accepted.



\subsection{Theoretical guarantees}

First, we formally relate the gain $g^\pi$ that we optimize for in \eqref{eq:CMDP-opt1} to the quantity of interest $\mathbb{E}^{p,\pi}[\tau]$.
\begin{lemma}\label{lem:gain2time}
For any stationary policy $\pi$, $\mathbb{E}^{p,\pi}[\tau] = \frac{K}{g^\pi}$.
\end{lemma} 
Lemma \ref{lem:gain2time} is a direct consequence of the fact that $\tau + K$ follows a negative binomial distribution with parameters $K$ and $1-g^\pi$, which are respectively the number of successes and the probability of failure, i.e. of rejecting a candidate under $\pi$. Note that this is only true because in our case the transition structure of the MDP ensures constant gain. A quick sanity check shows that if the agent systematically accepts all candidates, i.e. $g^\pi = 1$, then $\mathbb{E}^{p,\pi}[\tau] = K$, and that maximizing $g^\pi$ is equivalent to minimizing $\mathbb{E}^{p,\pi}[\tau]$. 

Then, we exhibit a bound on the representation loss incurred by following the stationary policy from the average-reward CMDP approach. Let $\tilde{d} = \sum_{i=1}^d (D_i - 1)$. Note that when all attributes are binary, $\tilde{d} = d$. 

\begin{proposition}\label{prop:hoeffding-loss}
Let $\pi^*$ be an optimal stationary policy for \eqref{eq:CMDP-opt1}. Let $\delta > 0$. Then, %$\mathbb{P}^\pi\left[\loss{C_\tau} \leq \sqrt{\frac{\log(\frac{2\tilde{d}}{\delta})}{2K}}\right] \geq 1 - \delta.$
\begin{align*}
    \mathbb{P}^{p,\pi^*}\left[\loss{C_\tau} \leq \sqrt{\frac{\log(\frac{2\tilde{d}}{\delta})}{2K}}\right] \geq 1 - \delta.
\end{align*}
\end{proposition}

All proofs are available in Appendix \ref{sec:proof-cmdp}.

The upper bound on the representation loss decreases with the committee size in $\sqrt{1/K}$. This shows that the stationary policy $\optpi$ works well for larger committees, although it acts independently from previously accepted candidates. The intuition is that for larger committees, adding a candidate has less impact on the current representation vector. It was the opposite in Example \ref{ex:small-committee} where the goal was to recruit a very small committee of size $K=4.$

%\virginie{[TODO] Compare with the $1/K + \tol$ from \greedyalg, where $\tol$ (probably) has a strong impact on the sample complexity $\tau$, but this I still need to prove.}



